Go for a Walk and Arrive at the Answer: Reasoning Over Paths in Knowledge Bases using Reinforcement Learning

Knowledge bases (KB), both automatically and manually constructed, are often incomplete --- many valid facts can be inferred from the KB by synthesizing existing information. A popular approach to KB completion is to infer new relations by combinatory reasoning over the information found along other paths connecting a pair of entities. Given the enormous size of KBs and the exponential number of paths, previous path-based models have considered only the problem of predicting a missing relation given two entities or evaluating the truth of a proposed triple. Additionally, these methods have traditionally used random paths between fixed entity pairs or more recently learned to pick paths between them. We propose a new algorithm MINERVA, which addresses the much more difficult and practical task of answering questions where the relation is known, but only one entity. Since random walks are impractical in a setting with combinatorially many destinations from a start node, we present a neural reinforcement learning approach which learns how to navigate the graph conditioned on the input query to find predictive paths. Empirically, this approach obtains state-of-the-art results on several datasets, significantly outperforming prior methods.

==> sections/NELL_experiments.tex <==
We test our model on many popular benchmark KB query answering datasets and compare our model with current state-of-the-art methods on those benchmarks. As noted by previous work \citep{e2e_diff_proving,deeppath,daschains,yang2017differentiable}, often the reasoning chains required to answer queries in KB is not too long (restricted to 3 or 4 hops). Therefore to test if our model can learn long reasoning paths, we test our model on a synthetic grid world dataset. We also show that our model is extensible and can be easily adapted to handle natural language queries by testing on a standard QA dataset.
\subsection{Data}
\begin{center}
\begin{table*}[t]
\begin{center}
\begin{tabular}{c c c c c}\hline
Dataset & \#entities & \#relations & \#facts & \#queries\\\hline
Countries & 272 & - & 1158 & -\\
\textsc{UMLS} & 135 & 49 & 6.5k & - \\t
Kinship & 104 & 26 & 10686 & - \\\hline
\textsc{WN18RR} & - & - & - & - \\
\textsc{Nell-995} & 75,492 & 200 & 154,213 & - \\
\textsc{FB15k-237} & 14,505 & 237 & 310,116 & -\\\hline
WikiMovies & 43,230 & 9 & 196,453 & 10,000\\\hline
\end{tabular}
\caption{Statistics of various datasets used in experiments.}
\label{tab:data_stats}
\end{center}
\end{table*}
\end{center}
We test our model on the following KB query answering datasets. (a) \textsc{Countries} \citep{complex}, (b) Alyawarra kinship (\textsc{Kinship}), (c) Unified Medical Language Systems (\textsc{UMLS}) \citep{kok2007} (d) \textsc{WN18RR} \citep{dettmers2017}, (e) \textsc{NELL-995} \citep{deeppath}, (f) \textsc{FB15k-237} \citep{fb15k-237}. The first three datasets are carefully designed to explicitly test the logical rule learning and reasoning capabilities of link prediction models. We also test our model on existing large and challenging KG datasets ((d) - (f)). \textsc{WN18RR} and \textsc{FB15k-237} are created from the original \textsc{WordNet18} and \textsc{Freebase15k} counter parts by removing test triples which could be answered trivially, hence making the 
\begin{center}
\begin{table*}[ht]
\begin{center}
\begin{tabular}{c c c c c c c}\hline
\multicolumn{2}{c}{Corpus} & Metric & \multicolumn{4}{c}{Model}\\
&  &  & \textbf{ComplEx} & \textbf{NTP} & \textbf{NTP-}$\lambda$ & \textbf{Our Model}\\\hline
& & MRR & 0.58 & 0.57 & 0.60 & - \\
& & \textsc{hits}@1 & 0.47 & 0.47 & 0.51 & \textbf{0.53} \\
\textsc{umls}& & \textsc{hits}@3 & 0.63 & 0.60 & 0.64 & \textbf{0.67} \\
& & \textsc{hits}@10 & 0.80 & 0.79 & \textbf{0.81} & \textbf{0.81} \\\hline
& & MRR & 0.46 & 0.36 & 0.48 & - \\
& & \textsc{hits}@1 & 0.34 & 0.24 & 0.39 & \textbf{0.46} \\
\textsc{Kinship}& & \textsc{hits}@3 & 0.49 & 0.40 & 0.47 & \textbf{0.62} \\
& & \textsc{hits}@10 & 0.74 & 0.60 & 0.71 & \textbf{0.76} \\\hline
\end{tabular}



==> sections/data.tex <==
We test our model on the following query answering datasets. (a) \textsc{countries} \citep{complex}, (b) Alyawarra kinship (\textsc{kinship}), (c) Unified Medical Language Systems (\textsc{umls}) \citep{kok2007} (d) \textsc{wn18rr} \citep{dettmers2017}, (e) \textsc{nell-995}, (f) \textsc{fb}15k-237 (g) WikiMovies \citep{kvmemnn}. We also test on a synthetic grid world dataset released by \citet{yang2017differentiable} to evaluate the model's ability to learn longer paths.

The \textsc{countries} dataset is carefully designed to explicitly test the logical rule learning and reasoning capabilities of link prediction models. The dataset has 3 tasks (S1-3 in table ~\ref{tab:countries}) each requiring reasoning steps of increasing length and difficulty (see \citet{e2e_diff_proving} for more details about the tasks). We also test our model on existing large and challenging KG datasets ((d) - (f)). \textsc{wn18rr} is  created from the original \textsc{wordnet18} dataset by removing test triples which can be answered trivially, making the datasets more realistic and challenging. Additionally, we test our model on a question answering dataset - WikiMovies \citep{kvmemnn} where the query is in \emph{natural language} but the answers can be found in an accompanying KB. Table \ref{tab:data_stats} report the various statistics of the datasets.

==> sections/task.tex <==
% \todoiz{Do we need this section? Possibly merge with intro?}


% \todoiz{We can also generalize this and bring in category theory: KB are quivers, then we want to explore some patterns ... but its tricky}

